Statistical field theory for neural networks

These notes attempt a self-contained introduction into statistical field theory applied to neural networks of rate units and binary spins. The presentation consists of three parts: First, the introduction of fundamental notions of probabilities, moments, cumulants, and their relation by the linked cluster theorem, of which Wick's theorem is the most important special case; followed by the diagrammatic formulation of perturbation theory, reviewed in the statistical setting. Second, dynamics described by stochastic differential equations in the Ito-formulation, treated in the Martin-Siggia-Rose-De Dominicis-Janssen path integral formalism. With concepts from disordered systems, we then study networks with random connectivity and derive their self-consistent dynamic mean-field theory, explaining the statistics of fluctuations and the emergence of different phases with regular and chaotic dynamics. Third, we introduce the effective action, vertex functions, and the loopwise expansion. These tools are illustrated by systematic derivations of self-consistency equations, going beyond the mean-field approximation. These methods are applied to the pairwise maximum entropy (Ising spin) model, including the recently-found diagrammatic derivation of the Thouless-Anderson-Palmer mean field theory.

==> tex/aux_field.tex <==

\section{Appendix: Auxiliary field formulation}

We here aim at a more general approach to the problem of a systematic
fluctuation expansion of a theory with the action $S[x,f[x]]$, where
we are interested in approximations of $y=f[x]$. As an example, we
may think of the disorder-averaged generating functional \eqref{eq:Zbar_pre}
of a network of the form
\begin{align}
S[\bx,\tbx,Q_{1}[\bx]] & =S_{0}[\bx,\tbx]+\frac{1}{2}\,\iint\,\sum_{i}\tx_{i}(t)\tx_{i}(s)\,Q_{1}(t,s)\,dt\,ds\label{eq:example_scs}\\
Q_{1}[\bx] & =\frac{g^{2}}{N}\sum_{i}\phi(x_{i}(t))\phi(x_{i}(s)).\nonumber 
\end{align}
Here we would identify $x=(\bx,\tbx)$ and $y=Q_{1}[\bx]$, so $f=Q_{1}$.

We proceed with this more abstract formulation. The generating functional
of $y$ then has the form
\begin{align*}
Z[j] & =\int\D x\,\exp(S[x,f[x]]+j^{\T}f(x)).
\end{align*}
The problem that prevents us from applying the standard formalism
is here that the integral is over the field $x$ not $f(x)$. So we
need to find a way to perform this substitution.

To have $y$ represented explicitly, we introduce the constraint $y=f[x]$
by a functional Dirac $\delta$ as
\begin{align}
Z[j] & =\int Dy\,\int\D x\,\delta[f[x]-y]\,\exp(S[x,y]+j^{\T}y)\nonumber \\
 & =\int Dy\,\int D\ty\,\int\D x\,\exp(\ty^{\T}(f[x]-y)+S[x,y]+j^{\T}y).\label{eq:Z_j_aux}
\end{align}

We may find an interpretation of the latter equation by rearranging
the integrals to get
\begin{align*}
W[j,\tj] & =\ln\int Dy\,\int D\ty\,\exp(-\ty^{\T}y+W[\ty|y]+j^{\T}y+\tj^{\T}\ty)\\
W[\ty|y] & :=\ln\int\D x\,\exp(S[x,y]+\ty^{\T}f[x]).
\end{align*}
This form shows that the latter line can be seen as the conditioned
cumulant generating functional, given the value $y$ inserted for
$f[x]$. Here $\ty$ plays the role of the source field.

In the example \eqref{eq:example_scs} given above, $W[\ty|y]$ provides
us with the statistics of $Q_{1}$ given we assume a fixed value $Q_{1}^{\ast}$
for $Q_{1}$. The self-consistency is ensured by the term $-\ty^{\T}y$
in the outer integral. We have here introduced a second source field
$\tj$ coupling to $\ty$.

We can now apply the standard procedure to obtain a systematic fluctuation
expansion of $y$ and $\ty$ by defining the vertex-generating functional
\begin{align*}
\Gamma[y^{\ast},\ty^{\ast}] & =\sup_{j,\tj}\,j^{\T}y^{\ast}+\tj^{\T}\ty^{\ast}-W[j,\tj].
\end{align*}
To lowest order in the fluctuations we hence get
\begin{align*}
\Gamma_{0}[y^{\ast},\ty^{\ast}] & =-S[y^{\ast},\ty^{\ast}]\\
 & =\ty^{\ast\T}y^{\ast}-W[\ty^{\ast}|y^{\ast}].
\end{align*}
We therefore obtain from the equation of state the pair of equations
\begin{align*}
j & =\frac{\delta\Gamma_{0}[y^{\ast},\ty^{\ast}]}{\delta y^{\ast}}=\ty^{\ast}-\frac{\delta}{\delta y^{\ast}}W[\ty^{\ast}|y^{\ast}].\\
\tj & =\frac{\delta\Gamma_{0}[y^{\ast},\ty^{\ast}]}{\delta\ty^{\ast}}=y^{\ast}-\frac{\delta}{\delta\ty}W[\ty^{\ast}|y^{\ast}].
\end{align*}
In the example \eqref{eq:example_scs}, the normalization of the $W[\ty|y]$
does not depend on the choice of $y$. Hence, for vanishing sources
the first equation yields $\ty^{\ast}=0$. The second equation provides
us with
\begin{align*}
y^{\ast} & =\langle y|y^{\ast}\rangle-\tj,
\end{align*}
where the conditional expectation value is understood as the mean
of $y$ given we fix $y=y^{\ast}$ in the second argument of the action
$S[x,y^{\ast}]$. In the example \eqref{eq:example_scs} this equation
would amount to the saddle point equations
\begin{align*}
Q_{1}^{\ast}(t,s) & =\frac{g^{2}}{N}\sum_{i}\langle\phi(x_{i}(t))\phi(x_{i}(s))\rangle_{Q_{1}^{\ast}},\\
\langle\circ\rangle_{Q_{1}^{\ast}} & =\frac{\int Dx\,\circ\,\exp(S_{0}[x]+\frac{1}{2}\,\tx^{\T}Q_{1}^{\ast}\tx)}{\int Dx\,\exp(S_{0}[x]+\frac{1}{2}\,\tx^{\T}Q_{1}^{\ast}\tx)}.
\end{align*}
Going to higher orders we note that the term $\ty^{\T}y$ only contributes
up to the Gaussian fluctuations. All interaction vertices will be
given by derivatives of $W[\ty|y]$ only. At second order we get
\begin{align*}
-S[y^{\ast},\ty^{\ast}]^{(2)} & =\left(\begin{array}{cc}
0 & 1-\frac{\delta^{2}}{\delta y^{\ast}\delta\ty^{\ast}}W[\ty^{\ast}|y^{\ast}]\\
1-\frac{\delta^{2}}{\delta\ty^{\ast}\delta y^{\ast}}W[\ty^{\ast}|y^{\ast}] & -\frac{\delta^{2}}{\delta\ty^{\ast2}}W[\ty^{\ast}|y^{\ast}]
\end{array}\right).
\end{align*}
Here the mixed derivatives $\frac{\delta^{2}}{\delta y^{\ast}\delta\ty^{\ast}}W[\ty^{\ast}|y^{\ast}]$
are response functions of $\langle y\rangle$ with respect to an infinitesimal
perturbation of $y$ mediated by the dynamics of $x$. The upper left
element $-\frac{\delta^{2}}{\delta y^{\ast2}}W[\ty^{\ast}|y^{\ast}]=0$
vanishes, because the normalization of $W[\ty|y^{\ast}]$ is independent
of the choice of $y^{\ast}$ in the second argument. The lower right
element is the negative variance of $y$ for given and fixed $y^{\ast}$.

The bare propagators for $y$ and $\ty$ therefore obey the set of
equations $-S^{(2)}\Delta=1$, so in particular it follows explicitly
\begin{align*}
\left(1-\frac{\delta^{2}}{\delta y^{\ast}\delta\ty^{\ast}}W[\ty^{\ast}|y^{\ast}]\right)\,\Delta_{\ty y} & =1\\
\left(1-\frac{\delta^{2}}{\delta\ty^{\ast}\delta y^{\ast}}W[\ty^{\ast}|y^{\ast}]\right)\,\Delta_{yy}-\frac{\delta^{2}}{\delta\ty^{\ast2}}W[\ty^{\ast}|y^{\ast}]\,\Delta_{\ty y} & =0.
\end{align*}
Multiplying the second equation from left with $\Delta_{y\ty}$ and
using the first line (with interchanged order of time indices and
hence $\ty\leftrightarrow y$), we get
\begin{align*}
\Delta_{\ty y} & =\left(1-\frac{\delta^{2}W[\ty^{\ast}|y^{\ast}]}{\delta y^{\ast}\delta\ty^{\ast}}\right)^{-1},\\
\Delta_{yy} & =\Delta_{y\ty}\,\frac{\delta^{2}W[\ty^{\ast}|y^{\ast}]}{\delta\ty^{\ast2}}\,\Delta_{\ty y},\\
\Delta_{\ty\ty} & =0.
\end{align*}
We see that, in line with the fluctuation expansion, all properties
are calculated at the point $y^{\ast}$.




==> tex/phi34_gamma_explicit.tex <==

\subsection{Problems\label{sec:Problems_phi34_gamma}}

\subsection*{a) Second-order approximation of $\Gamma$ for the ``$\phi^{3}+\phi^{4}$''-theory}

Determine diagrammatically all contributions at second order to $\Gamma$,
extending the results of \prettyref{sub:Example-Vertex-function-phi34}.
You may make use of the connected diagrams contributing to $W$ in
\prettyref{sec:Example_Connecteddiagrams_phi34}. (6 points)

\subsection*{b) Explicit calculation of $\Gamma$ for the ``$\phi^{3}$''-theory}

For the action \eqref{def_S_phi34}, setting $\beta=0$, calculate
the effective action $\Gamma$ explicitly in a perturbation expansion
up to second order in $\epsilon$ as the Legendre transform of $W(j)$.
Your calculation may follow along the lines of the general calculation
in \prettyref{sub:Explicit-cancellation-reducible}:
\begin{enumerate}
\item Start with the result \eqref{Gamma0_phi34}, valid to lowest order.
\item Determine all diagrams correcting $W$ to first and second order.
\item Perform the Legendre transform by determining the $j$ that maximizes
\prettyref{eq:Gamma_decomp-2}; convince yourself that you only need
$j$ correct up to first order in $\epsilon$, if $\Gamma$ is supposed
to be correct up to second order.
\item Insert the found $j$ into the definition of $\Gamma$ \prettyref{eq:Gamma_decomp-2}
and see how two one-line reducible diagrams produced at second order
are canceled.
\end{enumerate}
(8 points)

\subsection*{c) Effective equation of motion}

We here study the stochastic differential \eqref{nonlin_sde}

\begin{align}
dx(t)+x(t)\,dt & =\frac{\epsilon}{2!}x^{2}(t)\,dt+dW(t)\label{eq:nonlin_sde-1}
\end{align}
from the lecture and want to derive the effective equation of motion
for the mean value of $x^{\ast}(t)=\langle x(t)\rangle$ from the
equation of state \eqref{equation_of_state} expressed with help of
the effective action. First approximate the effective action to lowest
order by \prettyref{eq:Gamma0_Gauss} as $\Gamma_{0}[x^{\ast},\tx^{\ast}]=-S[x^{\ast},\tx^{\ast}]$
(1 point). We know from \prettyref{sec:Vanishing-response-field}
that the true mean value of $\langle\tx(t)\rangle\equiv0\quad\forall t$.
Show that this is indeed a solution of the equation of state (2 points).
So we only need to consider the single equation
\begin{align}
\tj(t) & =\frac{\delta\Gamma[x^{\ast},\tx^{\ast}]}{\delta\tx^{\ast}(t)}.\label{eq:eq_state_MSR}
\end{align}
We now want to determine the fluctuation corrections in perturbation
theory, according to \prettyref{sec:Vertex-functions-Gaussian}. 

Show by functional Taylor expansion \prettyref{eq:func_Taylor} of
$\Gamma[x,\tx]$ in the field $x$, that the effective equation of
motion can be written with the help of the vertex functions, the derivatives
of $\Gamma$, as
\begin{align*}
\tj(t) & =-(\partial_{t}+1)\,x^{\ast}(t)+\frac{\epsilon}{2!}x^{\ast2}(t)+\sum_{n=0}^{\infty}\frac{1}{n!}\,\prod_{l=1}^{n}\{\int dt_{l}\}\,\frac{\delta\Gamma_{V}[x^{\ast}=0,\tx^{\ast}=0]}{\delta\tx^{\ast}(t)\,\delta x^{\ast}(t_{1})\cdots\delta x^{\ast}(t_{n})}\,x^{\ast}(t_{1})\cdots x^{\ast}(t_{n}).
\end{align*}
(2 points). We now would like to determine the fluctuation corrections
up to the linear order in $x^{\ast}$ to get the effective equation
of motion
\begin{align}
\tj(t) & =-(\partial_{t}+1)\,x^{\ast}(t)+\frac{\delta\Gamma_{V}}{\delta\tx^{\ast}(t)}+\int\,dt^{\prime}\,\frac{\delta\Gamma_{V}}{\delta\tx^{\ast}(t)\delta x^{\ast}(t^{\prime})}\,x^{\ast}(t^{\prime})+O(\left(x^{\ast}\right)^{2}).\label{eq:eff_eq_motion}
\end{align}
Such an approximation would, for example, tell us how the system relaxes
back from a small perturbation away from $x^{\ast}=0$. The latter
integral term is a time-non-local, but linear indirect self-feedback
due to the fluctuations. 

Use the rules explained in \prettyref{sec:Vertex-functions-Gaussian}
and in \prettyref{sec:Perturbation-theory-for-MSR} to compute all
corrections to the effective equation of motion with one and two interaction
vertices. The result \prettyref{eq:correction_mean} may be useful
for the correction to the constant value $x^{\ast}$. The calculation
of the correction that is linear in $x^{\ast}$ may be easier in time
domain, using \prettyref{eq:free_covariance-1-1} and \prettyref{eq:free_response}
with $m=-1$. (4 points).

\ifthenelse{\boolean{includesolutions}}{

\subsection{Solutions}

\subsection*{a) Second order approximation of $\Gamma$ for the ``$\phi^{3}+\phi^{4}$''-theory}

At second order we have (using the results from Sec. \ref{sec:Example_Connecteddiagrams_phi34}
and noting that \prettyref{eq:second_order_phi34_var3} is not 1PI
and therefore drops out) 
\begin{align}
\Diagram{\vertexlabel_{x^{\ast}}{g}{}f{fl}{}{flu}{}f}
 & =4\cdot3\cdot2\,\frac{\epsilon^{2}}{2}\,\frac{\alpha}{3!}\,\frac{\beta}{4!}\,x^{\ast}\label{eq:second_order_phi34_var_1-1}\\
\nonumber \\
\Diagram{\vertexlabel_{x^{\ast}}{g}{}f0{fl}{}{flu}{}f0g\vertexlabel_{x^{\ast}}}
 & =3\cdot3\cdot2\,\frac{\epsilon^{2}}{2}\,\left(\frac{\alpha}{3!}\right)^{2}\frac{\left(x^{\ast}\right)^{2}}{2!}\label{eq:phi34_gamma_non_cancel}\\
\nonumber \\
\Diagram{\vertexlabel_{x^{\ast}}{g}{}f{fl}{}{flu}{}fg\vertexlabel_{x^{\ast}}}
 & =4\cdot4\cdot3\cdot2\,\frac{\epsilon^{2}}{2}\,\left(\frac{\beta}{4!}\right)^{2}\frac{\left(x^{\ast}\right)^{2}}{2!}\label{eq:second_order_phi34_var_2-1}\\
\nonumber \\
\Diagram{\vertexlabel^{x^{\ast}}gd & f0{fl}{}{flu}{}f0f0{fl}{}{flu}{}f0\\
\vertexlabel^{x^{\ast}}gu
}
 & =4\cdot3\cdot4\cdot3\,\frac{\epsilon^{2}}{2}\,\left(\frac{\beta}{4!}\right)^{2}\frac{\left(x^{\ast}\right)^{2}}{2!}\label{eq:second_order_phi34_var4-1}\\
\nonumber \\
\Diagram{\vertexlabel^{x^{\ast}}gd & f0{fl}{}{flu}{}f0g\vertexlabel^{x^{\ast}}\\
\vertexlabel^{x^{\ast}}gu
}
 & =4\cdot3\cdot3\cdot2\,\frac{\epsilon^{2}}{2}\,\frac{\alpha}{3!}\,\frac{\beta}{4!}\,\frac{\left(x^{\ast}\right)^{3}}{3!}\nonumber \\
\nonumber \\
\Diagram{\vertexlabel^{x^{\ast}}gd & f0{fl}{}{flu}{}f0gu\vertexlabel^{x^{\ast}}\\
\vertexlabel^{x^{\ast}}gu & f0f0gd\vertexlabel^{x^{\ast}}
}
 & =4\cdot3\cdot4\cdot3\cdot2\,\frac{\epsilon^{2}}{2}\,\frac{\alpha}{3!}\,\frac{\beta}{4!}\,\frac{\left(x^{\ast}\right)^{4}}{4!}.\nonumber 
\end{align}
In addition we get so called \textbf{vacuum diagrams} (without external
legs), such as
\begin{align}
\Diagram{{fl}{}{flu}{}f0f0{fl}{}{flu}{}f0}
 & =3\cdot\epsilon\frac{\beta}{4!},\nonumber \\
\nonumber \\
\Diagram{f{fl}{}{flu}{}f}
 & =3\cdot2\cdot\frac{\epsilon^{2}}{2}\,\left(\frac{\alpha}{3!}\right)^{2},\label{eq:vaccuum_phi34}
\end{align}
which can be dropped, because they do not have any $x^{\ast}$-dependence
and hence do not contribute to the vertex functions.

\subsection*{b) Explicit calculation of $\Gamma$ for the ``$\phi^{3}$''-theory}

To see that indeed all non 1PI graphs cancel, we determine an approximation
of $W(j)$ and find the value $j$ at which the supremum in \eqref{eq:def_gamma}
is attained. To lowest order we have \eqref{eq:Gamma0_phi34}. To
first order we get the corrections

\begin{align}
\Diagram{\vertexlabel_{j}{f}{}f0{fl}{}{flu}{}f0}
= & 3\cdot\,j\,\epsilon\frac{\alpha}{3!}=\epsilon\frac{\alpha}{2}\,j.\label{eq:first_order_phi43_1-1}\\
\nonumber 
\end{align}
In addition, we of course have the bare interaction vertices connected
to external sources, i.e. a contribution to the third cumulant
\begin{align*}
\Diagram{\vertexlabel^{j}fdf\vertexlabel_{j}\\
\vertexlabel^{j}fu
}
 & =3\cdot2\cdot\epsilon\frac{\alpha}{3!}\,\frac{j^{3}}{3!}=\epsilon\frac{\alpha}{3!}\,j^{3}.
\end{align*}
We note that by \eqref{eq:cumulant_Taylor} the $n$-th derivative
by $j$ comes with a factor $1/n!$. The corrections at second order
in $\epsilon$ are

\begin{align}
\Diagram{\vertexlabel_{j}{f}{}f0{fl}{}{flu}{}f0f\vertexlabel_{j}}
 & =3\cdot3\cdot2\,\frac{\epsilon^{2}}{2}\,\left(\frac{\alpha}{3!}\right)^{2}\,\frac{j^{2}}{2!}=\frac{1}{8}\,\epsilon^{2}\alpha^{2}\,j^{2}\nonumber \\
\nonumber \\
\Diagram{\vertexlabel^{j}fd & ff0{fl}{}{flu}{}f0\\
\vertexlabel^{j}fu
}
 & =3\cdot3\cdot2\cdot2\,\frac{\epsilon^{2}}{2}\,\left(\frac{\alpha}{3!}\right)^{2}\,\frac{j^{2}}{2!}=\frac{1}{4}\,\epsilon^{2}\alpha^{2}\,j^{2}\label{eq:phi34_gamma_cancel1}\\
\nonumber \\
\Diagram{\vertexlabel^{j}fd & ffu\vertexlabel^{j}\\
\vertexlabel^{j}fu & f0fd\vertexlabel^{j}
}
 & =3\cdot3\cdot4\cdot3\cdot2\,\frac{\epsilon^{2}}{2}\,\left(\frac{\alpha}{3!}\right)^{2}\,\frac{j^{4}}{4!}=\frac{1}{8}\,\epsilon^{2}\alpha^{2}\,j^{4}.\label{eq:phi34_gamma_cancel2}
\end{align}
We want to see how the latter non-1PI diagram gets canceled by performing
the Legendre transform. We first note that we only need to determine
the shift $j_{V}$ until first order in $\epsilon$, because the shift
cancels to linear order from $(j_{0}+j_{V})^{\T}x^{\ast}-W_{0}(j_{0}+j_{V})$,
since $j_{0}$ maximizes the expression. A shift of second order would
hence only contribute at forth order to $\Gamma$. So we have

\begin{align*}
W_{0}(j) & =\frac{1}{2}\,j^{2}\\
W_{1}(j) & =\epsilon\alpha\left(\frac{1}{2}j+\frac{1}{3!}j^{3}\right)\\
W_{2}(j) & =\frac{1}{8}\,\epsilon^{2}\alpha^{2}\,j^{2}+\frac{1}{4}\epsilon^{2}\alpha^{2}\,j^{2}+\frac{1}{8}\,\epsilon^{2}\alpha^{2}\,j^{4}.
\end{align*}
We need to maximize
\begin{align*}
\frac{\partial}{\partial j}\left(j^{\T}x^{\ast}-W_{0}(j)-W_{1}(j)\right) & \stackrel{!}{=}0.\\
x^{\ast}-j-\epsilon\alpha\left(\frac{1}{2}+\frac{1}{2}j^{2}\right) & =0.
\end{align*}
We only need to solve the latter equation correct up to first order
in $\epsilon$. We may hence replace $j$ in the term quadratic in
$\epsilon$ by the lowest order solution $j_{0}=x^{\ast}$, because
any correction would be of second order and higher. So we have
\begin{align*}
x^{\ast}-j-\epsilon\alpha\frac{1}{2}\left(1+\left(x^{\ast}\right)^{2}\right) & =O(\epsilon^{2}).\\
j & =x^{\ast}-\epsilon\alpha\frac{1}{2}\left(1+\left(x^{\ast}\right)^{2}\right)+O(\epsilon^{2}).\\
 & =j_{0}+j_{1}.
\end{align*}
Comparing to \eqref{eq:Gamma_1_phi34}, we see that $j_{1}=\Gamma^{(1)}(x^{\ast})$
holds. The correction term $j_{1}\propto\epsilon$ causes new terms
\begin{align*}
\Gamma(x^{\ast}) & =\underbrace{(j_{0}+j_{1}+j_{2})\,x^{\ast}-W_{0}(j_{0}+j_{1}+j_{2})}_{j_{0}x^{\ast}-W_{0}(j_{0})-\frac{1}{2}j_{1}^{\T}W_{0}^{(2)}(j_{0})j_{1}+O(\epsilon^{3})}\\
 & -W_{1}(j_{0}+j_{1})\\
 & -W_{2}(j_{0})+O(\epsilon^{3}).
\end{align*}
The identification in the first line is correct because we expand
$W_{0}$ about $j_{0}$ and therefore, because $j_{0}$ is defined
by fulfilling $W_{0}^{\left(1\right)}\left(j_{0}\right)=x^{\ast}$,
which leads to the cancellation of the term $\left(j_{1}+j_{2}\right)x^{\ast}$
with $W_{0}^{\left(1\right)}\left(j_{0}\right)\left(j_{1}+j_{2}\right)$.
That is why we do not have to calculate $j_{2}$ (and in general $j$
only up to order $n-1$ of we want to calculate $\Gamma$ correctly
up to order $n$). Furthermore, we identify $\Gamma_{0}\left(x^{\star}\right)=j_{0}x^{\star}-W_{0}\left(j_{0}\right)$.
With 
\begin{align*}
-W_{1}(j_{0}+j_{1}) & =-W_{1}(j_{0})-W_{1}^{(1)}(j_{0})\,j_{1}+O(\epsilon^{3})\\
 & =-W_{1}(j_{0})+\epsilon\alpha\frac{1}{2}\left(1+\left(x^{\ast}\right)^{2}\right)\,\epsilon\alpha\frac{1}{2}\left(1+\left(x^{\ast}\right)^{2}\right)\\
-\frac{1}{2}\,j_{1}^{\T}W_{0}^{(2)}(j_{0})\,j_{1} & =-\frac{1}{2}\,\left(\epsilon\alpha\frac{1}{2}\left(1+\left(x^{\ast}\right)^{2}\right)\right)^{2}
\end{align*}
we see that we may combine both terms and have
\begin{align*}
\Gamma(x^{\ast}) & =\underbrace{\frac{1}{2}\left(x^{\ast}\right)^{2}}_{\Gamma_{0}}-\underbrace{\epsilon\alpha x^{\ast}\left(\frac{1}{2!}+\frac{1}{3!}\left(x^{\ast}\right)^{2}\right)}_{-W_{1}(j_{0})}\\
 & +\underbrace{\frac{1}{2}\,\left(\epsilon\alpha\frac{1}{2}\left(1+\left(x^{\ast}\right)^{2}\right)\right)^{2}}_{=-\frac{1}{2}\,j_{1}^{\T}W_{0}^{(2)}(j_{0})\,j_{1}-W_{1}^{(1)}(j_{0})\,j_{1}}\\
 & \underbrace{-\frac{1}{8}\epsilon^{2}\alpha^{2}\,\left(x^{\ast}\right)^{2}-\frac{1}{4}\,\epsilon^{2}\alpha^{2}\,\left(x^{\ast}\right)^{2}-\frac{1}{8}\,\epsilon^{2}\alpha^{2}\,\left(x^{\ast}\right)^{4}}_{-W_{2}(j_{0})}\\
 & =\frac{1}{2}\left(x^{\ast}\right)^{2}-\epsilon\alpha x^{\ast}\left(\frac{1}{2!}+\frac{1}{3!}\left(x^{\ast}\right)^{2}\right)\\
 & +\frac{1}{2}\,\left(\frac{\epsilon\alpha}{2}\right)^{2}+\underline{\frac{1}{4}\,\left(\epsilon\alpha\right)^{2}\,\left(x^{\ast}\right)^{2}}+\underline{\frac{1}{2}\,\left(\frac{\epsilon\alpha}{2}\right)^{2}\left(x^{\ast}\right)^{4}}\\
 & -\frac{1}{8}\epsilon^{2}\alpha^{2}\,\left(x^{\ast}\right)^{2}\underline{-\frac{1}{4}\,\epsilon^{2}\alpha^{2}\,\left(x^{\ast}\right)^{2}}-\underline{\frac{1}{8}\,\epsilon^{2}\alpha^{2}\,\left(x^{\ast}\right)^{4}}.
\end{align*}
The first term in the third line is the diagram \eqref{eq:phi34_gamma_non_cancel}
obtained before, while the contributions of the two diagrams \eqref{eq:phi34_gamma_cancel1}
and \eqref{eq:phi34_gamma_cancel2} canceled from the final expression,
because they are not 1PI. We also note that we got a constant contribution
in addition, corresponding to the vacuum diagram \eqref{eq:vaccuum_phi34}

\subsection*{c) Effective equation of motion}

We here study the example \eqref{eq:nonlin_sde}

\begin{align}
dx(t)+x(t)\,dt & =\frac{\epsilon}{2!}x^{2}(t)\,dt+dW(t)\label{eq:nonlin_sde-1-2}
\end{align}
from the lecture and want to derive the effective equation of motion
for the mean value of $x^{\ast}(t)=\langle x(t)\rangle$ from the
equation of state \eqref{eq:equation_of_state} expressed with help
of the effective action. First approximate the effective action to
lowest order by \prettyref{eq:Gamma0_Gauss} as $\Gamma_{0}[x^{\ast},\tx^{\ast}]=-S[x^{\ast},\tx^{\ast}]$
(1 point). We know from \prettyref{sec:Vanishing-response-field}
that the true mean value of $\langle\tx(t)\rangle\equiv0\quad\forall t$.
Show that this is indeed a solution of the equation of state (2 points).
So we only need to consider the single equation
\begin{align}
\tj(t) & =\frac{\delta\Gamma[x^{\ast},\tx^{\ast}]}{\delta\tx^{\ast}(t)}.\label{eq:eq_state_MSR-1}
\end{align}
We now want to determine the fluctuation corrections in perturbation
theory, according to \prettyref{sec:Vertex-functions-Gaussian}. 

Show by functional Taylor expansion \prettyref{eq:func_Taylor} of
$\Gamma[x,\tx]$ in the field $x$, that the effective equation of
motion can be written with the help of the vertex functions in the
form
\begin{align*}
\tj(t) & =-(\partial_{t}+1)\,x^{\ast}(t)+\frac{\epsilon}{2!}x^{\ast2}(t)+\sum_{n=0}^{\infty}\frac{1}{n!}\,\prod_{l=1}^{n}\{\int dt_{l}\}\,\frac{\delta\Gamma_{V}[x^{\ast}=0,\tx^{\ast}=0]}{\delta\tx^{\ast}(t)\,\delta x^{\ast}(t_{1})\cdots\delta x^{\ast}(t_{n})}\,x^{\ast}(t_{1})\cdots x^{\ast}(t_{n}).
\end{align*}
(2 points). We now would like to determine the fluctuation corrections
up to the linear order in $x^{\ast}$, namely
\begin{align}
\tj(t) & =-(\partial_{t}+1)\,x^{\ast}(t)+\frac{\delta\Gamma_{V}}{\delta\tx^{\ast}(t)}+\int\,dt^{\prime}\,\frac{\delta\Gamma_{V}}{\delta\tx^{\ast}(t)\delta x^{\ast}(t^{\prime})}\,x^{\ast}(t^{\prime})+O(\left(x^{\ast}\right)^{2}).\label{eq:eff_eq_motion-1}
\end{align}
Such an approximation would, for example, tell us how the system relaxes
back from a small perturbation away from $x^{\ast}=0$. The latter
integral term is a time-non-local, but linear indirect self-feedback
due to the fluctuations. How does the appearing vertex function $\Gamma_{V,\tx x}^{(2)}$
relate to the self-energy \prettyref{eq:def_self_energy}? (1 point)

Use the rules explained in \prettyref{sec:Vertex-functions-Gaussian}
and in \prettyref{sec:Perturbation-theory-for-MSR} to compute all
corrections to \eqref{eq:eff_eq_motion-1} with one and two interaction
vertices. The result \prettyref{eq:correction_mean} may be useful
for the correction to the constant value $x^{\ast}$. The calculation
of the correction that is linear in $x^{\ast}$ may be easier in time
domain, using \prettyref{eq:free_covariance-1-1} and \prettyref{eq:free_response}
with $m=-1$. (4 points).

The contribution $\frac{\delta\Gamma_{V}}{\delta\tx^{\ast}(t)}$ has
a single amputated leg $\tx$ and follows as
\begin{align*}
\Diagram{\vertexlabel_{\tilde{X}(\omega)}gVf0flVfluVf0}
= & \frac{\epsilon}{2!}\int\,\frac{d\omega_{2}}{2\pi}\frac{d\omega_{3}}{2\pi}\,\delta(\omega+\omega_{2}+\omega_{3})\,\delta(\omega_{2}+\omega_{3})\,(2\pi)\,\left(-i\omega_{2}+1\right)^{-1}D\left(i\omega_{2}+1\right)^{-1}\,\\
= & \frac{\epsilon}{2!}\frac{1}{2\pi}\,\delta(\omega)\,\int\,d\omega_{2}\,\left(-i\omega_{2}+1\right)^{-1}D\left(i\omega_{2}+1\right)^{-1}\\
= & \delta(\omega)\,\frac{\alpha D}{4},
\end{align*}
where the calculation is the same as in \prettyref{eq:correction_mean}.
We hence get a positive offset $\frac{\alpha D}{4}$. The other diagram
is
\begin{align*}
\Diagram{\vertexlabel_{\tilde{x}(t)}gVf0flVfluf0gV\vertexlabel_{x(s)}f0}
 & =-\frac{1}{2!}\,\left(\frac{\epsilon}{2!}\right)^{2}\cdot2\cdot2\cdot2\cdot\Delta_{x\tx}(t,s)\Delta_{xx}(t,s)\\
 & =\alpha^{2}\,H(t-s)\,e^{-(t-s)}\,\frac{D}{2}\,e^{-|t-s|}\\
 & =\frac{\alpha^{2}\,D}{2}\,H(t-s)\,e^{-2(t-s)},
\end{align*}
where we used the expressions for $\Delta_{x\tx}$ and $\Delta_{xx}$
in time domain \prettyref{eq:free_covariance-1-1} and \prettyref{eq:free_response}
with $m=-1$. We hence get the effective equation of motion to linear
order in $x^{\ast}$
\begin{align*}
\tj(t) & =-(\partial_{t}+1)\,x^{\ast}(t)+\frac{\epsilon D}{4}+\frac{\epsilon^{2}\,D}{2}\,\int_{-\infty}^{t}\,e^{-2(t-s)}\,x^{\ast}(s)\,ds,
\end{align*}
where we also dropped the term $\frac{\epsilon}{2!}x^{\ast2}(t)$,
because it is quadratic in $x^{\ast}$. The form shows that the system
acquires memory of the past, so it is not a Markov process anymore.
Still, the evolution only depends on the past activity. Differentiating
another time by $t$ transforms the equation of motion into an ordinary
differential equation of second order.

}{}.

